Peak Time-Windowed Risk Estimation of Stochastic Processes

This paper develops a method to upper-bound extreme-values of time-windowed risks for stochastic processes. Examples of such risks include the maximum average or 90% quantile of the current along a transmission line in any 5-minute window. This work casts the time-windowed risk analysis problem as an infinite-dimensional linear program in occupation measures. In particular, we employ the coherent risk measures of the mean and the expected shortfall (conditional value at risk) to define the maximal time-windowed risk along trajectories. The infinite-dimensional linear program must then be truncated into finite-dimensional optimization problems, such as by using the moment-sum of squares hierarchy of semidefinite programs. The infinite-dimensional linear program will have the same optimal value as the original nonconvex risk estimation task under compactness and regularity assumptions, and the sequence of semidefinite programs will converge to the true value under additional properties of algebraic characterization. The scheme is demonstrated for risk analysis of example stochastic processes.

==> macros/jared_tac_macros.tex <==
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{hyperref}
\hypersetup{colorlinks=true, linkcolor=black}
%Single Symbols
\newcommand{\R}{\mathbb{R}} 
\newcommand{\K}{\mathbb{K}} 
\newcommand{\C}{\mathbb{C}} 
\newcommand{\N}{\mathbb{N}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Lie}{\mathcal{L}} 
\newcommand{\ks}{\mathcal{K}} 
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zt}{\mathcal{Z}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\s}{\mathcal{S}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\scL}{\mathscr{L}}

\newcommand{\ts}{\mathcal{T}}
\newcommand{\gs}{\mathcal{G}}
\newcommand{\es}{\mathcal{E}}
\newcommand{\vs}{\mathcal{V}}

\newcommand{\urg}[1]{{\color{red} #1}}


%reinserting macros
\newcommand{\A}{\mathcal{A}}
% \newcommand{\R}{\mathcal{R}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\rbm}{\rev{\bm}}
\newcommand{\psd}{\mathbb{S}}
\newcommand{\cs}{\mathcal{C}}

%Paired Commands
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\Tr}{\textrm{Tr}(}{)}
\DeclarePairedDelimiter{\rank}{\textrm{rank}(}{)}
\DeclarePairedDelimiter{\diag}{\textrm{diag}(}{)}
\DeclarePairedDelimiter{\vvec}{\textrm{vec}(}{)}
\DeclarePairedDelimiter{\mmat}{\textrm{mat}(}{)}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\supp}{\textrm{supp}(}{)}
\DeclarePairedDelimiter{\Mp}{\mathcal{M}_+(}{)}

\newcommand{\weak}{\overset{\ast}{\rightharpoonup}}
% \usepackage{amsthm}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{conj}{Conjecture}[section]
\newtheorem{exmp}{Example}[section]
\newtheorem{remark}{Remark}
\newtheorem{problem}{Problem}

==> sections/biography.tex <==
% \vspace{0.5in}

%\newpage

% \vspace{1cm}
% \newpage
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/jared_kdd_small.jpg}}]{Jared Miller}  is currently a Post-Doctoral Researcher at the Automatic Control Laboratory (IfA) at ETH Z\"{u}rich, in the research group of Prof. Roy S. Smith. He received his B.S. and M.S. degrees in Electrical Engineering from Northeastern University in 2018, and his Ph.D. degree from Northeastern University in 2023 under the advisorship of Mario Sznaier (Robust Systems Laboratory). He is a recipient of the 2020 Chateaubriand Fellowship from the Office for Science Technology of the Embassy of France in the United States. He was given an Outstanding Student Paper award at the IEEE Conference on Decision and Control in 2021 and in 2022. His research interests include large-scale convex optimization,  measure theory, nonlinear dynamics, and power systems.
\end{IEEEbiography}

% % \newpage
% \InsertBoxL{0}{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/NiklasSchmid_TAC.png}}\par
% \textbf{Niklas Schmid} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/NiklasSchmid_TAC.png}}]{Niklas Schmid} is a Ph.D. student at the Automatic Control Laboratory (IfA), ETH Z\"{u}rich, Switzerland, in the research group of Professor John Lygeros, which he joined in 2021. He received his M.Sc. and B.Sc. degree in Medical Engineering Science at the University of L\"{u}beck, Germany, in 2021 and 2019, respectively. In 2020 and 2021 he worked on the control of electrosurgical generators at Olympus Surgical Technologies Europe in Berlin, Germany. His research focuses on the control of stochastic systems under safety constraints.
\end{IEEEbiography}

% \InsertBoxL{0}{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/tacchi.png}}\par
% \textbf{Matteo Tacchi} 

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/tacchi.png}}]{Matteo Tacchi} received a Master's degree in Mathematics from Paris VI University in 2016, and a Ph.D. degree in control theory from Toulouse University in 2021. During his Ph.D., he addressed large scale set approximation problems through convex optimization methods, with application to approximating stability regions of dynamical systems. From 2021 to 2023, he was a postdoctoral fellow with the Automatic Control Laboratory, École Polytechnique Fédérale de Lausanne, working on model and data based optimization for control. He is currently a junior researcher in CNRS GIPSA-lab.
\end{IEEEbiography}
% % \vspace{0.5in}
% % % \newpage
% % % \newpage

% \InsertBoxL{0}{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/didier2019.jpg}}\par
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/didier2019.jpg}}]{Didier Henrion} is currently a CNRS ``Directeur de Recherche" (senior researcher) at LAAS in the research group POP. He is also holding a secondary appointment as a Professor at the Department of Automatic Control of the Faculty of Electrical Engineering of the Czech Technical University in Prague.
He received the Masters’ and Engineer’s degrees from the National Institute for Applied
Sciences (INSA), Toulouse, France, in 1994, a
Ph.D. degree from the Academy of Sciences
of the Czech Republic, Prague, in 1998, and
a Ph.D. degree from INSA in 1999, all in the
area of control. Since 2000 Didier Henrion has
been a researcher of CNRS (French National
Center for Scientific Research) at LAAS (Laboratory of Analysis and Architecture of Systems).
\end{IEEEbiography}

% % \newpage
% \vspace{0.5in}
% \InsertBoxL{0}{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{example-image-a}}\par
% \textbf{Roy S. Smith}  
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/rsmith.jpg}}]{Roy S. Smith} is a professor of Electrical Engineering at the Swiss Federal Institute of Technology (ETH), Zürich. Prior to joining ETH in 2011, he was on the faculty of the University of California, Santa Barbara, from 1990 to 2010. His Ph.D. is from the California Institute of Technology (1990) and his undergraduate degree is from the University of Canterbury (1980) in his native New Zealand. He has been a long-time consultant to the NASA Jet Propulsion Laboratory and has industrial experience in automotive control and power system design. His research interests involve the modeling, identification, and control of uncertain systems. Particular control application domains of interest include chemical processes, flexible structure vibration, spacecraft and vehicle formations, aerodynamic control of kites, automotive engines, Mars aeromaneuvering entry design, building and energy hub control, and thermoacoustic machines. He is a Life Fellow of the IEEE and the IFAC, an Associate Fellow of the AIAA, and a member of SIAM.
\end{IEEEbiography}

==> sections/contributions_over.tex <==
Portions of this work were submitted to the 2024 IEEE Conference on Decision and Control in \urg{[placemark for CDC citation]}. Contributions in this work beyond the conference version in \urg{[placemark for CDC citation]} include:
\begin{itemize}
    \item A consideration of continuous-time and discrete-time stochastic processes in dynamics rather than \acp{ODE}.
    \item Risk functionals $\mathcal{R}$ beyond the mean.
    \item Proofs of strong duality and convergence.
    \item Additional examples.
\end{itemize}

To the best of our knowledge, the time-windowed risk estimation problem for stochastic processes has not previously been addressed in the literature. The closest existing work to this research (beyond the conference work in \urg{[placemark for CDC citation]}) is the prior article \cite{miller2023chancepeak} (which included the first and third author), which focuses on the instantaneous risk estimation problem. Treating the time-windowed risk estimation  Problem \ref{prob:risk_window} using measure \ac{LP} techniques requires nontrivial manipulations and extensions as compared to the method of \cite{miller2023chancepeak} (the introduction of the augmented time $s$ with accessory support constraints).

==> sections/extensions.tex <==
\section{Extensions}
\label{sec:extensions}
\urg{Other uncertainties in dynamics (robustness, switching)

Other risk measures.


Effect of MDP discretization rather than Moment-SOS.


}

\subsection{Time Windowed Peak Markov Decision Process [Preliminary sketch]}
The preceeding occupation measure based analysis of problem \eqref{eq:risk_window} naturally extends to classical linear programming approaches for the optimal control of discrete time Markov Decision Processes. This allows to extend our formulation to the analysis of and controller synthesis for non-autonomous systems with a minimum time windowed peaks. Let $\mathcal{X}$ and $\mathcal{U}$ denote two Borel subspaces of complete seperable metric spaces denoting the state and input space and let them be equipped with Borel $\sigma$-algebras $\mathcal{B(X)}, B(U)$, respectively. The stochastic kernel $T:\mathcal{B(X)}\times\mathcal{X}\times\mathcal{U}$ yields the stochastic dynamics; At a given time-step $k\in\mathbb{N}$, state $x_k\in\mathcal{X}$ and input $u_k\in\mathcal{U}$ the consecutive state $x_{k+1}$ at time-step $k+1$ is rendered from the kernel $x_{k+1}\sim T(\cdot|x_k,u_k)$. We further define Markov policies $\pi=\{\mu_0,\dots, \mu_N\}$ as a sequence of Borel-measurable stochastic kernels $\mu_k:\mathcal{X}\times\mathcal{B(U)}\rightarrow[0,1]$. We denote the set of all Markov policies as $\Pi$. Given a policy $\pi$, kernel $T$, initial state $\delta_0$ a unique occupation measure is defined [cite Abate2008 Paper]. 

\color{red} Put Assumptions here. We might need weakly continuous kernels, compact X, U etc., let's discuss. \color{black}


In the following, we aim to minimize the expected window averaged peak over all possible windows $s\in[h,N]$ via a suitable policy $\pi\in\Pi$. Consider the linear program
\begin{align}
    &\inf_{\mu_{0:N}\in\mathcal{M}_+(\mathcal{X}\times\mathcal{U}),\gamma\in\mathbb{R}_{\geq 0}}
    &&\gamma   \nonumber
    \\
    &\text{s.t.} &&\hspace{-2cm} \int_{\mathcal{U}}\mu_{k+1}(A,du) = \int_{A,\mathcal{U}}\mu_k(x,u)T(A|dx,du),  \nonumber\\
    &&&\hspace{-2cm}\int_{\mathcal{X},\mathcal{U}}\mu_k(dx,du)=1 \label{eq_mdp_lp}\\
    &&&\hspace{-2cm}\mu_0 = \delta_0 \nonumber \\
    &&&\hspace{-2cm} \gamma \geq\sum_{k=s-h}^s\int_{\mathcal{X}\times\mathcal{U}} p(x)\mu_k(dx,du) \nonumber
\end{align}
where the constraints hold for all $k\in[N-1], s\in[h,N]$ and all $A\in\mathcal{B(X)}$. 
\begin{lem}
    The infimum in Problem \eqref{eq_mdp_lp} is attained.
    \label{lem_mdp_lp_attainability}
\end{lem}
\begin{proof}
    tbd
\end{proof}
\begin{thm}
    Let $\gamma^{\star}$ and $\mu_{0:N}^{\star}$ denote an optimal argument in Problem \eqref{eq_mdp_lp}. Then, $\gamma^{\star}$ is the minimum time window averaged peak, which is achieved by a policy $\pi\in\Pi$.
\end{thm}
\begin{proof}
    Optimal arguments $\gamma^{\star}$ and $\mu_{0:N}^{\star}$ for Problem \eqref{eq_mdp_lp} are guaranteed to exist by Lemma \ref{lem_mdp_lp_attainability}. Further, the existence of a policy $\pi\in\Pi$ with the occupation measure $\mu_{0:N}^{\star}$ follows by [cite Lerma]. By feasibility of the occupation measure associated to $\pi$ in Problem \eqref{eq_mdp_lp} we have $\mathbb{E}_{\delta_0,\pi}\left[\sum_{k=s-h}^sp(x_k)\right] = \sum_{k=s-h}^s\int_{\mathcal{X}\times\mathcal{U}} p(x)\mu_k(dx,du) \leq \gamma$ for all $s\in[h,N]$. 

    Lastly, there does not exist a policy $\pi\in\Pi$ that yields a lower window averaged peak than $\gamma^{\star}$. For the sake of contradiction, assume there does exist a policy $\pi\in\Pi$ with associated occupation measure $\mu_{0:N}$ and maximum time windowed averaged peak $\gamma<\gamma^{\star}$. Then, $\gamma,\mu_{0:N}$ is feasible in Problem \eqref{eq_mdp_lp}. However, this is a contradiction by optimality of $\gamma^{\star}$ in \eqref{eq_mdp_lp}.
\end{proof}

Whenever $\mathcal{X}$ and $\mathcal{U}$ are continuous Problem \eqref{eq_mdp_lp} is infinite dimensional. To resort to a tractable formulation, gridding approximations are popularly applied. \color{red}(Explicit error bounds are available under Lipschitz continuity assumptions on the function $p$ and the kernel density. I would have to dig them up to find them if we want to include them.)\color{black}
